Studying Aspects of the Early Universe with Primordial Black Holes

This thesis by publication is devoted to the study of aspects of the early universe in the context of primordial black hole (PBH) physics. Firstly, we review the fundamentals of the early universe cosmology and we recap the basics of the PBHs physics. In particular, we propose a refinement in the determination of the PBH formation threshold, a fundamental quantity in PBH physics, in the context of a time-dependent equation-of-state parameter. Afterwards, we briefly present the theory of inflationary perturbations, which is the theoretical framework within which PBHs are studied in this thesis. Then, in the second part of the thesis, we review the core of the research conducted within my PhD, in which aspects of the early universe and the gravitational wave physics are combined with the physics of PBHs. Moreover, aspects of the PBH gravitational collapse process are studied in the presence of anisotropies. Specifically, we study PBHs produced from the preheating instability in the context of single-field inflation. Interestingly, we find that PBHs produced during preheating can potentially dominate the universe's content and drive reheating through their evaporation. Then, we focus on the scalar induced second-order stochastic gravitational wave background (SGWB) induced from Poisson energy density fluctuations of ultralight PBHs. By taking then into account gravitational wave backreaction effects we set model-independent constraints on the initial abundance of ultralight PBHs as a function of their mass. Afterwards, we study in a covariant way the anisotropic spherical gravitational collapse of PBHs during a radiation-dominated era in which one can compute the PBH formation threshold as a function of the anisotropy. Finally, we summarize our research results by discussing future prospects opened up as a result of the research work conducted within this thesis.

==> PhD Thesis/newcommands.tex <==
%edition
%\newcommand{\ie}{\textsl{i.e.~}}
\newcommand{\ie}{{i.e.~}}
\newcommand{\cf}{\textsl{cf.~}}
%\newcommand{\eg}{\textsl{e.g.~}}
\newcommand{\eg}{e.g.~}
\newcommand{\etal}{\textsl{et al.~}}
%\newcommand{\apriori}{\textsl{a priori~}}
\newcommand{\apriori}{{a priori~}}
\newcommand{\etc}{\textsl{etc.~}}

% PBH Phi symbols
\newcommand{\OmegaPBH}{\Omega_{\mathrm{PBH}}}
\newcommand{\OmegaGW}{\Omega_{\mathrm{GW}}}
\newcommand{\rhoGW}{\rho_{\mathrm{GW}}}
\newcommand{\rhoend}{\rho_{\mathrm{end}}}
\newcommand{\rhoreh}{\rho_{\mathrm{reh}}}
\newcommand{\rhorad}{\rho_{\mathrm{rad}}}
\newcommand{\rhoBBN}{\rho_{\mathrm{BBN}}}
\newcommand{\rhoinstab}{\rho_{\mathrm{instab}}}
\newcommand{\phiend}{\phi_{\text{end}}}
\newcommand{\phiwell}{\phi_{\text{well}}}		% Was phi_wall/phi_barrier
\newcommand{\phiuv}{\phi_{\text{uv}}}			% was phi_wall
\newcommand{\phisr}{\phi_{\text{sr}}}
%\newcommand{\phisto}{\phi_{\text{sto}}}
\newcommand{\phisto}{\Delta\phiwell}
\newcommand{\phicl}{\phi_{\mathcal{P}_{\zeta}|_{\mathrm{cl}}>1}}		% {\phi_{\text{cl}}}
\newcommand{\N}{\mathcal{N}}

% New definition of square root:
% renames \sqrt as \oldsqrt
\let\oldsqrt\sqrt
% it defines the new \sqrt in terms of the old one
\def\sqrt{\mathpalette\DHLhksqrt}
\def\DHLhksqrt#1#2{%
\setbox0=\hbox{$#1\oldsqrt{#2\,}$}\dimen0=\ht0
\advance\dimen0-0.2\ht0
\setbox2=\hbox{\vrule height\ht0 depth -\dimen0}%
{\box0\lower0.4pt\box2}}

%math function
\newcommand{\mean}[1]{\left\langle #1 \right\rangle}
%\newcommand{\order}[1]{\mathcal{O}\!\left(#1\right)}
\newcommand{\Li}[1]{\mathrm{Li}_{#1}}
\DeclareMathOperator{\Ei}{Ei}
\DeclareMathOperator{\Ai}{Ai}
\DeclareMathOperator{\Bi}{Bi}
%\DeclareMathOperator{\erf}{erf}
\DeclareMathOperator{\erfc}{erfc}
%\newcommand{\tr}{\mathrm{Tr}}

%larger math symbols
\newcommand{\largemathxl}[1]{{\mathlarger{#1}}}
\newcommand{\largemathxxl}[1]{{\mathlarger{\mathlarger{#1}}}}
\newcommand{\largemathxxxl}[1]{{\mathlarger{\mathlarger{\mathlarger{#1}}}}}
\newcommand{\mathlargerxxxxl}[1]{{\mathlarger{\mathlarger{\mathlarger{\mathlarger{#1}}}}}}
\newcommand{\mathlargerxxxxxl}[1]{{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{#1}}}}}}}
\newcommand{\mathlargerxxxxxxl}[1]{{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{#1}}}}}}}}
\newcommand{\mathlargerxxxxxxxl}[1]{{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{#1}}}}}}}}}
\newcommand{\mathlargerxxxxxxxxl}[1]{{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{#1}}}}}}}}}}
\newcommand{\mathlargerxxxxxxxxxl}[1]{{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{#1}}}}}}}}}}}
\newcommand{\mathlargerxxxxxxxxxxl}[1]{{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{\mathlarger{#1}}}}}}}}}}}}

%alias
\newcommand{\lta}{\lesssim}
\newcommand{\gta}{\gtrsim}
%differential d
%\newcommand{\dd}{\mathrm{d}}
%e function
%\newcommand{\ee}{\mathrm{e}}
\newcommand{\ee}{e}


%style
\newcommand{\sss}[1]{{\scriptscriptstyle{#1}}}
\newcommand{\boldmathsymbol}[1]{{\ensuremath{\boldsymbol{#1}}}}

%SR, USR
\newcommand{\SR}{{{}_\mathrm{SR}}}
\newcommand{\USR}{{{}_\mathrm{USR}}}

\newcommand{\uPl}{\mathrm{Pl}}
\newcommand{\uin}{\mathrm{in}}
\newcommand{\umin}{\mathrm{min}}
\newcommand{\umax}{\mathrm{max}}
\newcommand{\uend}{\mathrm{end}}
\newcommand{\uei}{\mathrm{ei}}
\newcommand{\uini}{\mathrm{ini}}
\newcommand{\ueff}{\mathrm{eff}}
\newcommand{\uinf}{\mathrm{inf}}
\newcommand{\ureh}{\mathrm{reh}}
\newcommand{\urad}{\mathrm{rad}}
\newcommand{\utop}{\mathrm{top}}
\newcommand{\ucri}{\mathrm{cri}}
\newcommand{\ucl}{\mathrm{cl}}
\newcommand{\unuc}{\mathrm{nuc}}
\newcommand{\uobs}{\mathrm{obs}}
\newcommand{\ulim}{\mathrm{lim}}
\newcommand{\uphys}{\mathrm{phys}}
\newcommand{\uPgiP}{\mathrm{(gi)}}
\newcommand{\ue}{\mathrm{e}}
\newcommand{\uc}{\mathrm{c}}
\newcommand{\ub}{\mathrm{b}}
\newcommand{\us}{\mathrm{s}}
\newcommand{\uS}{\mathrm{S}}
\newcommand{\uM}{\mathrm{M}}
\newcommand{\uPSP}{(\uS)}
\newcommand{\uV}{\mathrm{V}}
\newcommand{\uT}{\mathrm{T}}
\newcommand{\uPTP}{(\uT)}
\newcommand{\uE}{\mathrm{E}}
\newcommand{\usssTE}{\sss{\uT \uE}}
\newcommand{\usssS}{\sss{\uS}}

\newcommand{\lo}{\sss{\mathrm{LO}}}
\newcommand{\nlo}{\sss{\mathrm{NLO}}}
\newcommand{\nnlo}{\sss{\mathrm{NNLO}}}

\newcommand{\usssPSP}{\sss{\uPSP}}
\newcommand{\usssT}{\sss{\uT}}
\newcommand{\usssPTP}{\sss{\uPTP}}
\newcommand{\usssPMoneP}{\sss{(\uM=1)}}
\newcommand{\usssPl}{\sss{\uPl}}
\newcommand{\usssRH}{\ureh}
\newcommand{\usssV}{\sss{\uV}}
\newcommand{\usssE}{\sss{\uE}}
\newcommand{\nS}{n_\usssS}
\newcommand{\nT}{n_\usssT}
\newcommand{\alphaS}{\alpha_\usssS}
\newcommand{\alphaT}{\alpha_\usssT}
\newcommand{\zero}{{_0}}
\newcommand{\one}{{_1}}
\newcommand{\two}{{_2}}
\newcommand{\udm}{\mathrm{dm}}
\newcommand{\ud}{\mathrm{d}}
\newcommand{\muS}{\mu_\usssS}
\newcommand{\muT}{\mu_\usssT}
\newcommand{\muST}{\mu_{\usssS,\usssT}}
\newcommand{\uRL}{\mathrm{RL}}
\newcommand{\uNL}{\mathrm{NL}}
\newcommand{\uwkb}{\mathrm{WKB}}

\newcommand{\bmk}{\boldmathsymbol{k}}
\newcommand{\bmx}{\boldmathsymbol{x}}

\newcommand{\calH}{\mathcal{H}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calI}{\mathcal{I}}

\newcommand{\setR}{\mathbb{R}}
\newcommand{\setC}{\mathbb{C}}

\newcommand{\Rea}{\Re \mathrm{e}\,}
\newcommand{\Ima}{\Im \mathrm{m}\,}


%units
\newcommand{\eV}{\mathrm{eV}}
\newcommand{\keV}{\mathrm{keV}}
\newcommand{\MeV}{\mathrm{MeV}}
\newcommand{\GeV}{\mathrm{GeV}}
\newcommand{\TeV}{\mathrm{TeV}}
\newcommand{\cm}{\mathrm{cm}}
\newcommand{\g}{\mathrm{g}}
\newcommand{\km}{\mathrm{km}}
\renewcommand{\sec}{\mathrm{s}}
\newcommand{\pc}{\mathrm{pc}}
\newcommand{\kpc}{\mathrm{kpc}}
\newcommand{\Mpc}{\mathrm{Mpc}}
\newcommand{\K}{\mathrm{K}}

% General Cosmology

\newcommand{\Hu}{\mathcal{H}}
\newcommand{\Ka}{\mathcal{K}}
\newcommand{\Zed}{\mathcal{Z}}
\newcommand{\cs}{c_{_\mathrm{S}}}

%cosmo
\newcommand{\omegaT}{\omega_\usssT}
\newcommand{\omegaS}{\omega_\usssS}
\newcommand{\omegaST}{\omega_{\usssS, \usssT}}
\newcommand{\OmegaL}{\Omega_\Lambda}
\newcommand{\OmegaCDM}{\Omega_\udm}
\newcommand{\OmegaB}{\Omega_\ub}
\newcommand{\OmegaR}{\Omega_\gamma}
\newcommand{\Qrms}{Q_{\mathrm{rms-PS}}}
\newcommand{\wstate}{w}
\newcommand{\Mc}{M_\uc}
\newcommand{\potS}{U_{_\uS}}
\newcommand{\potT}{U_{_\uT}}

\newcommand{\mpl}{m_\usssPl}
\newcommand{\Mp}{M_\usssPl}


%inflation
\newcommand{\Hzero}{H_0}
\newcommand{\Hstar}{H_*}
\newcommand{\kstar}{k_*}
\newcommand{\Pstar}{P_*}
\newcommand{\astar}{a_*}
\newcommand{\Pnum}{P^{\usssPMoneP}}
\newcommand{\calNnuc}{\mathcal{N}^\unuc}
\newcommand{\calNend}{\mathcal{N}^\uend}
\newcommand{\calFnuc}{\mathcal{F}^\unuc}
\newcommand{\calFend}{\mathcal{F}^\uend}
\newcommand{\rRL}{r_\uRL}
\newcommand{\fnl}{f_\uNL}
\newcommand{\csini}{c_{\us \uini}}

\newcommand{\etastar}{\eta_*}
\newcommand{\nustar}{\nu_*}
\newcommand{\csstar}{c_{\us*}}
\newcommand{\epsonestar}{\epsilon_{1*}}
\newcommand{\epstwostar}{\epsilon_{2*}}
\newcommand{\epsthreestar}{\epsilon_{3*}}
\newcommand{\deltaonestar}{\delta_{1*}}
\newcommand{\deltatwostar}{\delta_{2*}}
\newcommand{\epsnstar}{\epsilon_{n*}}
\newcommand{\epsnponestar}{\epsilon_{n+1*}}
\newcommand{\xstar}{x_*}

\newcommand{\ustar}{u_*}
\newcommand{\wstar}{w_*}

\newcommand{\dia}{\sss{\diamond}}
\newcommand{\Hdia}{H_\dia}
\newcommand{\kdia}{k_\dia}
\newcommand{\etadia}{\eta_\dia}
\newcommand{\csdia}{c_{\us \dia}}
\newcommand{\epsonedia}{\epsilon_{1\dia}}
\newcommand{\epstwodia}{\epsilon_{2\dia}}
\newcommand{\epsthreedia}{\epsilon_{3\dia}}
\newcommand{\epsfourdia}{\epsilon_{4\dia}}
\newcommand{\epsfivedia}{\epsilon_{5\dia}}

\newcommand{\deltaonedia}{\delta_{1\dia}}
\newcommand{\deltatwodia}{\delta_{2\dia}}
\newcommand{\deltathreedia}{\delta_{3\dia}}
\newcommand{\deltafourdia}{\delta_{4\dia}}

\newcommand{\grav}{\star}
\newcommand{\Hgrav}{H_\grav}
\newcommand{\kgrav}{k_\grav}
\newcommand{\etagrav}{\eta_\grav}
\newcommand{\epsonegrav}{\epsilon_{1\grav}}
\newcommand{\epstwograv}{\epsilon_{2\grav}}

\newcommand{\aH}{\sss{\circledast}}
\newcommand{\kah}{k_\aH}
\newcommand{\etaah}{\eta_\aH}

\newcommand{\Dwkb}{D_{_\uwkb}}
\newcommand{\Awkb}{A_{_\uwkb}}
%\newcommand{\etaH}{\eta_{_{H}}}


%efolds
\newcommand{\efolds}{$e$-folds}
\newcommand{\efold}{$e$-fold}
\newcommand{\Nini}{N_\uini}
\newcommand{\Nend}{N_\uend}
\newcommand{\Nreh}{N_\ureh}
\newcommand{\Nstar}{N_*}
\newcommand{\Nzero}{N_\zero}
\newcommand{\Nstarnuc}{N_*^\unuc}
\newcommand{\Nstarend}{N_*^\uend}

%begin and end equations
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
%\newcommand{\bea}{\begin{eqnarray}}
%\newcommand{\eea}{\end{eqnarray}}
\newcommand{\bea}{\begin{equation}\begin{aligned}}
\newcommand{\eea}{\end{aligned}\end{equation}}



%figures size
\newlength{\wsingfig}
\setlength{\wsingfig}{0.99\textwidth}
\newlength{\wdblefig}
\setlength{\wdblefig}{0.49\textwidth}
\newlength{\wquadfig}
\setlength{\wquadfig}{0.249\textwidth}
\newlength{\wtriplefig}
\setlength{\wtriplefig}{0.333\textwidth}


% References
\newcommand{\Eq}[1]{Eq.~(\ref{#1})}
\newcommand{\Eqs}[1]{Eqs.~(\ref{#1})}
\newcommand{\Fig}[1]{Fig.~{\ref{#1}}}
\newcommand{\Figs}[1]{Figs.~{\ref{#1}}}
%\newcommand{\Ref}[1]{Ref.~{\cite{#1}}}
\newcommand{\Refs}[1]{Refs.~{\cite{#1}}}
\newcommand{\Sec}[1]{Sec.~\ref{#1}}
\newcommand{\Ch}[1]{Ch.~\ref{#1}}
\newcommand{\Secs}[1]{Secs.~\ref{#1}}
\newcommand{\Par}[1]{Par.~\ref{#1}}
\newcommand{\App}[1]{Appendix~\ref{#1}}
\newcommand{\Apps}[1]{Appendixes~\ref{#1}}

\newcommand{\mr}{\mathrm{r}}
\newcommand{\mt}{\mathrm{t}}

\newcommand{\mybox}{%
    \collectbox{%
        \setlength{\fboxsep}{7pt}%
        \fbox{\BOXCONTENT}%
    }%
}
